The Use of Presence Data in Modelling Demand for Transportation

We consider the applicability of the data from operators of cellular systems to modelling demand for transportation. While individual-level data may contain precise paths of movement, stringent privacy rules prohibit their use without consent. Presence data aggregate the individual-level data to information on the numbers of transactions at each base transceiver station (BTS) per each time period. Our work is aimed at demonstrating value of such aggregate data for mobility management while maintaining privacy of users. In particular, given mobile subscriber activity aggregated to short time intervals for a zone, a convex optimisation problem estimates most likely transitions between zones. We demonstrate the method on presence data from Warsaw, Poland, and compare with official demand estimates obtained with classical econometric methods.

==> text/additionalexperiments.tex <==

\section{Additional Computational Experiments}
\label{adexperiments}


To corroborate the bounds on the run-time presented in Theorems~\ref{thm:tracemax},
we present a results on a benchmark suggested by Cuturi \cite{Cuturi2013}. 
Specifically, we compare the methods of 
Rubner et al. \cite{RubnerTomasiGuibas2000},
Cuturi \cite{Cuturi2013},
Pele and Werman \cite{5459199}, referenced above, 
with our algorithm of Theorem~\ref{thm:tracemax}.
Notice that 
the implementation of ours and of \cite{Cuturi2013} are in Matlab, while 
the implementation of \cite{RubnerTomasiGuibas2000} and \cite{5459199}
are in C linked via MEX interfaces (\texttt{emd\_mex}, \texttt{emd\_hat\_gd\_metric}).
Also, the implementation of \cite{RubnerTomasiGuibas2000} is limited to $n=512$ or less, in practice.
As in \cite{Cuturi2013}, vectors in the $n$-dimensional simplex are generated 
for an increasing $n$.
The mean and standard deviations of the run-time for each method are plotted in Figure~\ref{fig:comptime}
as a function of dimension $n$. The asymptotes are clear.

\begin{figure}\centering
\centering
\includegraphics[width=.5\textwidth]{Pix/Computation_Times.pdf}
\caption{Run-time of EMD computations as a function of dimension $n$, with vectors sampled from the $n$-dimensional simplex
and mean and standard deviation displayed.}\label{fig:comptime}
\end{figure}

%\subsection{Run-time}


%Next, to compare the statistical performance ... 
%To train the SVM \eqref{SVM}, we use \texttt{libsvm}


%and generate random distance matrices $M$ by selecting $d$ points distributed with a spherical Gaussian in dimension $d/10$ to obtain enough variability in the distance matrix. $M$ is then divided by the median of its values, $\texttt{M=M/median(M(:))}$. Sinkhorn distances are implemented in matlab code (see Algorithm~\ref{alg:sk}) while \texttt{emd\_mex}, \texttt{emd\_hat\_gd\_metric} are mex/C files. 



%\subsection{MNIST Digits}\label{subsec:mnist}
%We test the performance of Sinkhorn distances on the MNIST digits\footnote{\texttt{http://yann.lecun.com/exdb/mnist/}} dataset, on which the ground metric has a natural interpretation in terms of pixel distances. Each digit is provided as a vector of intensities on a $20\times 20$ pixel grid. We convert each image into a histogram by normalizing each pixel intensity by the total sum of all intensities . 
%We consider a subset of $N$ points in the training set of the database, where $N$ ranges within $\{3,5,12,17,25\}\times 10^3$ datapoints. 
%
%\begin{figure}\centering
%%\fbox{\includegraphics[width=9cm]{res25000.pdf}}
%\caption{Average test errors with shaded confidence intervals. Errors are computed using 1/4 of the dataset for train and 3/4 for test. Errors are averaged over 4 folds $\times$ 6 repeats = 24 experiments.}
%\end{figure}
%\subsubsection{Experimental setting}  For each subset of size $N$, we provide mean and standard deviation of classification error using a 4 fold (3 test, 1 train) cross validation scheme repeated 6 times, resulting in 24 different experiments. We study the performance of different distances with the following parameter selection scheme: for each distance $d$, we consider the kernel $e^{-d/t}$, where $t>0$ is chosen by cross validation individually for each training fold within the set $\{1,q_{10}(d),q_{20}(d),q_{50}(d)\}$, where $q_s$ is the $s\%$ quantile of a subset of distances observed in the training fold. 
%We regularize non-positive definite kernel matrices resulting from this computation by adding a sufficiently large diagonal term. SVM's were run with \texttt{libsvm} (one-vs-one) for multiclass classification, the regularization constant $C$ being selected by 2 folds/2 repeats cross-validation on the training fold in the set $10^{-2:2:4}$
%
%\subsubsection{Distances} The Hellinger, $\chi_2$, Total Variation and squared Euclidean (Gaussian kernel) distances are used as such. We set the ground metric $M$ to be the Euclidean distance between the $20\times 20$ points in the grid, resulting in a $400\times 400$ distance matrix. We also tried to use Mahalanobis distances on this example with a positive definite matrix equal to \texttt{exp(-tM.\^{}2)}, \texttt{t>0},  as well as its inverse, with varying values of $t$ but none of the results proved competitive. For the Independence kernel, since any Euclidean distance matrix is valid, we consider $[m_{ij}^a]$ where $a\in\{0.01,0.1,1\}$ and choose $a$ by cross-validation on the training set. Smaller values of $a$ seem to be preferable. We select the entropic penalty $\lambda$ of Sinkhorn distances so that the matrix $e^{-\lambda M}$ is relatively diagonally dominant and the resulting transportation not too far from the classic optimal transportation. We select $\lambda$ for each training fold by internal cross-validation within $\{5,7,9,11\}\times 1/q_{50}(M)$ where $q_{50}(M)$ is the median distance between pixels on the grid. We set the number of fixed-point iterations to an arbitrary number of 20 iterations. In most (though not all) folds, the value $\lambda=9$ comes up as the best setting. The Sinkhorn distance beats by a safe margin all other distances, including the EMD.


